Factual Probing Is [MASK]: Learning vs. Learning to Recall

Petroni et al. (2019) demonstrated that it is possible to retrieve world facts from a pre-trained language model by expressing them as cloze-style prompts and interpret the model's prediction accuracy as a lower bound on the amount of factual information it encodes. Subsequent work has attempted to tighten the estimate by searching for better prompts, using a disjoint set of facts as training data. In this work, we make two complementary contributions to better understand these factual probing techniques. First, we propose OptiPrompt, a novel and efficient method which directly optimizes in continuous embedding space. We find this simple method is able to predict an additional 6.4% of facts in the LAMA benchmark. Second, we raise a more important question: Can we really interpret these probing results as a lower bound? Is it possible that these prompt-search methods learn from the training data too? We find, somewhat surprisingly, that the training data used by these methods contains certain regularities of the underlying fact distribution, and all the existing prompt methods, including ours, are able to exploit them for better fact prediction. We conduct a set of control experiments to disentangle "learning" from "learning to recall", providing a more detailed picture of what different prompts can reveal about pre-trained language models.

==> discussion.tex <==
%!TEX root = main.tex

\danqi{My main concern now is not about dense prompt vs fine-tuning, but whether dense prompt (maybe AutoPrompt is in a similar vein) is really a fair comparison to LAMA/LPAQA. The reason is that the model will pick up the distribution of objects (per relation) naturally from the training data. How can we avoid this? }
\zexuan{Maybe use macro accuracy (for each unique object, get an accuracy, and then average over all objects)? On the other hand, this distribution should be also the natural distribution in the Wikipedia. So the pre-trained model should have learned this during pre-trianing.}

\dan{1. AutoPrompt can also pick up the distribution of objects. The don't allow ``proper nouns and tokens that appear as gold objects'' in the prompts, but they can still find a set of input tokens so that $P(\text{object}|\text{prompt}_r)$ is somehow always just the most likely for that relation. 2. The LPAQA paper picks prompts for each relation based on accuracy on the training data, so I think it's exactly the same, it's just a worse approximation of $P(\text{object}|\text{prompt}_r)$. 3. I don't think this is a problem---what we }

\paragraph{RQ1.} What is a factual probe?

Probing is a method to gauge how much knowledge is already contained in pre-trained language models and can be used to compare different models. Most existing work on probing \ti{linguistic} knowledge usually trains a classifier on fixed language representations and uses the accuracy of the final probing task as the metric. However, this has been recently discussed that it is not easy to disentangle whether the knowledge is already contained in language models or learned by the probe, and thus the complexity of probes matters~\cite{hewitt2019designing}.

In another thread, researchers have attempted to probe how much factual knowledge (e.g., \ti{Barack Obama, born\_in, Hawaii}) is contained in pre-trained LMs ~\cite{petroni2019language}. Starting from manually templated prompts, it has been shown that better prompts can lead to better probing accuracy and this prompt can be either mined from text corpus~\cite{jiang2020can}, or even attained through gradient-based search~\cite{shin2020autoprompt}. Either approach has a learnable component that needs to make use of additional training data. Unlike general linguistic knowledge, factual knowledge only relies on the surface forms of subjects/objects and the general assumption is that if this training data has \ti{no overlap} with the evaluation data, any method using this data will not introduce any new factual knowledge during the probing process so the final accuracy can be used as a reliable estimate of what has been already stored in the weights of language models.

If this hypothesis is correct, we argue that we can directly optimize the input prompts or even fine-tune the full model (from this additional training data). \zexuan{even if the hypothesis is correct, it is not very natural for me that fine-tuning the full model is a probing task. I basically don't know how to make this point convincing.}

\danqi{Probing is not a task. Probing is a method/a way to measure how much knowledge is already contained in LMs. Why do you think dense prompt and fine-tuning have a fundamental difference? I don't see it.}

\zexuan{To make this point, I think we should study whether the intersection of predictions from prompt-based approaches and fine-tuning. Currently, the only evidence we have is that they can have the similar accuracy. If their predictions will also have much overlap, then I think it's another evidence.}  \danqi{Yes, I like the analysis of the intersection of predictions!}


\paragraph{RQ2.} Both OptPrompt and fine-tuning show that they can obtain ~49\% accuracy on LAMA - Does it mean that the model really know this portion of knowledge?

\begin{itemize}
    \item
        Experiment: Make harder constraints in training data. 1) Any subject in evaluation shouldn't appear in the training set. 2) Any training examples shouldn't have any lexical overlap with the evaluation subject. 3) Can we even constrain that the objects will not appear in the training set? If this is too harsh (e.g., your \ti{jazz} exmple), one possibility is to divide the examples into two subsets by grouping objects and only use the other subset to train. \zexuan{is this more suitable for RQ1? As we constrain that the model doesn't learn factual knowledge from the training set, we can say that the optimizing-based prompt and fine-tuning is a way to probe knowledge.} \danqi{I don't care it is RQ1 or RQ2. The paper may not be structured in this way. I think this part is the most crucial one. To have a setting that we can make sure that the model doesn't learn factual knowledge from the training set (or at least close to that).} \dan{I don't think it's a problem that the model can learn the distribution of objects, because we can just compare the model's prediction to a ``pick most common object'' baseline. Is there any other way that optimization could introduce new factual information?}
    \item
        How confident are these factual predictions? Do the models make some random guess sometimes? Can we use some calibration metrics (I put ECE in Table~\ref{tab:lama_results} for now)?
    \item
        Can we show that models don't know a fact? \danqi{Think about it.} \zexuan{given a query, if the current answer doesn't have a high rank (or a high probability) among all candidates (e.g., ``actor'', ``professor'', etc. for the occupation relation), then we may know the model doesn't know this fact.} \danqi{This is not convincing. Query is not fixed and can take many forms.} \dan{I think it's too confusing to ask about whether the model ``knows'' or doesn't ``know'' something---language models don't know anything, they assign probabilities to sequences of words. The only question we can really ask is whether it's possible to extract factual information from the model's parameters. From that perspective I'm not sure we can ever know whether some fact is not encoded, or our mechanism just fails to retrieve it. But we can measure how ``accessible'' a given fact is---if some facts can be retrieved by our method, and some can't, that might suggest that the facts the method doesn't retrieve are encoded in a less accessible form (if at all).} \danqi{I totally agree with what you said.}


\end{itemize}

\paragraph{RQ3.} Why do we care about probing of factual knowledge?
\begin{itemize}
    \item
        Comparison of different pre-trained language models Table~\ref{tab:comparison_lms}
    \item
        Show that this probing result can be correlated with downstream performance Table~\ref{tab:tacred_results} and this can explain why RoBERTa doesn't work well in TACRED.
        \zexuan{I think this is interesting. I also expect that entity only is consistent with probing results. But it seems that ``entity only'' is more like another probing task instead of a real downstream task. While for other settings (``context only'' and ``full''), it requires sentence understanding ability, not (only) the factual knowledge. So I am not sure what does that mean if a model can achieve higher performance in other settings. Can we draw any conclusion based on this?} \danqi{The point is to separate out the two factors and understand whether different models behave differently in the two. If the full model is a common choice for downstream tasks, then it is a combination of two types of knowledge. We just wanted to make this comparison here. BTW. This is what basically Tianyu's paper did, the bigger point is here to compare different LMs. }
\end{itemize}


==> figures/lama_hard.tex <==
\begin{figure}
    \centering
    \resizebox{0.9\columnwidth}{!}{%
    \includegraphics{figures/lama_hard.pdf}
    }
    \vspace{-0.5em}
    \caption{
    Accuracy on LAMA attributed to either LAMA-easy (facts that can be predicted in any of our random control settings), or LAMA-hard (the rest), micro-averaged over relations.
    The Oracle bar gives the relative size of each partition.
    %(LPAQA prompts are tuned on a different training set collected from Wikidata, which might have different class statistics.)
    }
    \label{fig:lama_hard}
\vspace{-1.3em}
\end{figure}


==> tables/breakdown.tex <==
%!TEX root = ../main.tex

\begin{table}[ht]
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{l | c c c c}
        \toprule
        Relations & Pre-trained & Rand E. & Rand M. & Majority \\
        \midrule
        P30 located in & 89.1 & 72.3 & 72.3 & 72.3 \\
        P176 produced by & 87.9 & 8.9 & 8.9 & 10.2 \\
        P103 name after & 74.1 & 24.8 & 0.3 & 60.1 \\
        P31 instance of & 65.7 & 8.9 & 8.7 & 15.3 \\
        P1001 legal in & 85.5 & 50.4 & 9.4 & 9.6 \\
        % \midrule
        % \multirow{4}{*}{\finetuning}
        % & P1376 capital of & 66.5 & 0.0 & 0.4 \\
        % & P463 member of & 62.2 & 59.1 & 57.3 \\
        % & P136 music genre & 62.6 & 54.8 & 55.4 \\
        % & P279 subclass of & 66.4 & 52.8 & 16.0 \\

        % \midrule
        % % \multirow{7}{*}{\autop} & P101. [X] works in the field of [Y] & 0.0/0.0 \\
        % % & P101. [X] works in the field of [Y] & 0.0/0.0 \\
        % % & P101. [X] works in the field of [Y] & 0.0/0.0 \\
        % % & \multicolumn{2}{c}{\ldots} \\
        % % & P101. [X] works in the field of [Y] & 0.0/0.0 \\
        % % & P101. [X] works in the field of [Y] & 0.0/0.0 \\
        % % & P101. [X] works in the field of [Y] & 0.0/0.0 \\
        % % \midrule
        % \multirow{7}{*}{\ours} & 
        % P30. [X] is located in [Y] & 89.1/3.7 \\
        % & P176. [X] is produced by [Y] & 87.9/0.3 \\
        % & P103. The native language of [X] is [Y] & 86.6/0.7 \\
        % & \multicolumn{2}{c}{\ldots} \\
        % & P108. [X] works for [Y] & 10.2/0.6 \\
        % & P530. [X] maintains diplomatic relations with [Y] & 3.1/0.0 \\
        % & P190. [X] and [Y] are twin cities & 3.0/2.9 \\
        % \midrule
        % \multirow{7}{*}{\finetuning} 
        % & P30. [X] is located in [Y] & 92.0/3.7 \\
        % & P176. [X] is produced by [Y] & 90.8/0.3 \\
        % & P103. The native language of [X] is [Y] & 86.3/0.7 \\
        % & \multicolumn{2}{c}{\ldots} \\
        % & P108. [X] works for [Y] & 11.0/-0.5 \\
        % & P190. [X] and [Y] are twin cities & 3.4/2.7 \\
        % & P530. [X] maintains diplomatic relations with [Y] & 3.2/-0.1\\
        \bottomrule
    \end{tabular}
    }
    \caption{Relation examples by different probing methods. See full breakdown accuracy in Appendix~\ref{appendix:breakdown}.
    %\dan{Do you think this would be easier to understand if it was more like Table~\ref{tab:train_test_overlap}? (1) Don't include gain, (2) use short labels (``occupation'') instead of prompts, (3) three columns: random bert, random embeddings, full bert. Then we can see which relations get the biggest improvements compared to the two controls.}
    %\zexuan{we may add more examples into the table. Do we need to show both {\ours} and {\finetuning} here in two blocks?}
    }
    \label{tab:breakdown}
\end{table}


% \begin{table}[ht]
%     \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{l | c r}
%         \toprule
%         Method & Relations & acc/$\mathcal{G}$ \\
%         \midrule
%         % \multirow{7}{*}{\autop} & P101. [X] works in the field of [Y] & 0.0/0.0 \\
%         % & P101. [X] works in the field of [Y] & 0.0/0.0 \\
%         % & P101. [X] works in the field of [Y] & 0.0/0.0 \\
%         % & \multicolumn{2}{c}{\ldots} \\
%         % & P101. [X] works in the field of [Y] & 0.0/0.0 \\
%         % & P101. [X] works in the field of [Y] & 0.0/0.0 \\
%         % & P101. [X] works in the field of [Y] & 0.0/0.0 \\
%         % \midrule
%         \multirow{7}{*}{\ours} & 
%         P30. [X] is located in [Y] & 89.1/3.7 \\
%         & P176. [X] is produced by [Y] & 87.9/0.3 \\
%         & P103. The native language of [X] is [Y] & 86.6/0.7 \\
%         & \multicolumn{2}{c}{\ldots} \\
%         & P108. [X] works for [Y] & 10.2/0.6 \\
%         & P530. [X] maintains diplomatic relations with [Y] & 3.1/0.0 \\
%         & P190. [X] and [Y] are twin cities & 3.0/2.9 \\
%         \midrule
%         \multirow{7}{*}{\finetuning} 
%         & P30. [X] is located in [Y] & 92.0/3.7 \\
%         & P176. [X] is produced by [Y] & 90.8/0.3 \\
%         & P103. The native language of [X] is [Y] & 86.3/0.7 \\
%         & \multicolumn{2}{c}{\ldots} \\
%         & P108. [X] works for [Y] & 11.0/-0.5 \\
%         & P190. [X] and [Y] are twin cities & 3.4/2.7 \\
%         & P530. [X] maintains diplomatic relations with [Y] & 3.2/-0.1\\
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{A list of relations by different probing methods.
%     \dan{Do you think this would be easier to understand if it was more like Table~\ref{tab:train_test_overlap}? (1) Don't include gain, (2) use short labels (``occupation'') instead of prompts, (3) three columns: random bert, random embeddings, full bert. Then we can see which relations get the biggest improvements compared to the two controls.}
%     }
%     \label{tab:breakdown}
% \end{table}

% \begin{table}
%     \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{l | cc cc cc | cc cc}
%         \toprule
%         Method & \multicolumn{2}{c}{$1-1$} & \multicolumn{2}{c}{$N-1$} & \multicolumn{2}{c}{$N-M$} & \multicolumn{2}{c}{relation1} & \multicolumn{2}{c}{relation2} \\
%         & Acc. & $\mathcal{G}$ & Acc. & $\mathcal{G}$ & Acc. & $\mathcal{G}$ & Acc. & $\mathcal{G}$ & Acc. & $\mathcal{G}$ \\
%         \midrule
%         $q(o)$ & & & & & & & & & &\\
%         $q(o|w_1)$  & & & & & & & & & &\\
%         {\autop}  & & & & & & & & & &\\
%         {\ours}  & & & & & & & & & &\\
%         {\finetuning}  & & & & & & & & & &\\
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{We break down the performance of three probes by T-REx relation type. Each column gives accuracy and information gain as a percentage relative to the control for either a category of relations or a particular representative relation. (``capital of'' is an example of a $1-1$ relation, ``place of birth'' is $N-1$, and ``shares border with'' is $N-M$.) We highlight two representative categories. For relation1, fine-tuning gives a large improvement in accuracy but a low information gain relative to the control, indicating that this relationship can be learned from the training data. relation2 had a relatively lower improvement in accuracy but a higher information gain, which suggests that some improvement is from information stored in the model's parameters.}
%     \label{tab:breakdown}
% \end{table}


==> tables/breakdown_full.tex <==
%!TEX root = ../main.tex

\begin{table*}[ht]
    \resizebox{2.\columnwidth}{!}{%
    \begin{tabular}{l | lr |rrr | rrr | r }
        \toprule
        \multirow{2}{*}{\tf{Relation}} &  \multicolumn{2}{c|}{{\bf LAMA (manual prompts)}} & \multicolumn{3}{c|}{{\bf \ours}} & \multicolumn{3}{c|}{{\bf \finetuning}} & \tf{Class} \\
         & Prompt & Acc & Acc & Rand E. & Rand M. & Acc & Rand E. & Rand M. & \tf{Prior}\\
        \midrule
P1001 & [X] is a legal term in [Y] . & 70.5 & 85.2 & 42.8 & 9.6 & 85.6 & 54.9 & 9.7 & 9.6 \\ 
P101 & [X] works in the field of [Y] . & 9.9 & 14.1 & 10.1 & 10.5 & 15.5 & 10.8 & 10.8 & 10.8 \\ 
P103 & The native language of [X] is [Y] . & 72.2 & 86.8 & 60.1 & 60.1 & 86.1 & 63.5 & 60.5 & 60.1 \\ 
P106 & [X] is a [Y] by profession . & 0.6 & 34.7 & 27.5 & 14.3 & 34.8 & 30.8 & 26.4 & 14.3 \\ 
P108 & [X] works for [Y] . & 6.8 & 11.5 & 8.9 & 6.3 & 10.2 & 9.1 & 9.4 & 7.8 \\ 
P127 & [X] is owned by [Y] . & 34.8 & 50.8 & 7.0 & 6.8 & 50.7 & 17.2 & 12.4 & 6.8 \\ 
P1303 & [X] plays [Y] . & 7.6 & 25.7 & 22.8 & 10.6 & 24.9 & 22.7 & 22.8 & 22.8 \\ 
P131 & [X] is located in [Y] . & 23.3 & 39.5 & 2.3 & 0.2 & 40.4 & 1.5 & 0.6 & 0.6 \\ 
P136 & [X] plays [Y] music . & 0.8 & 64.0 & 55.4 & 55.3 & 63.5 & 56.1 & 55.4 & 55.4 \\ 
P1376 & [X] is the capital of [Y] . & 73.9 & 57.9 & 0.0 & 0.0 & 62.7 & 0.0 & 0.0 & 0.4 \\ 
P138 & [X] is named after [Y] . & 61.6 & 74.6 & 3.9 & 1.6 & 75.7 & 50.8 & 1.6 & 1.6 \\ 
P140 & [X] is affiliated with the [Y] religion . & 0.6 & 71.7 & 53.7 & 53.7 & 77.6 & 53.7 & 53.7 & 53.7 \\ 
P1412 & [X] used to communicate in [Y] . & 65 & 76.2 & 27.7 & 25.3 & 76.3 & 28.0 & 28.2 & 20.6 \\ 
P159 & The headquarter of [X] is in [Y] . & 32.4 & 37.7 & 9.0 & 9.0 & 37.3 & 7.7 & 9.0 & 9 \\ 
P17 & [X] is located in [Y] . & 31.3 & 57.1 & 2.8 & 1.9 & 58.1 & 7.7 & 2.6 & 2.8 \\ 
P176 & [X] is produced by [Y] . & 85.6 & 89.5 & 8.9 & 8.9 & 90.4 & 80.0 & 70.2 & 8.9 \\ 
P178 & [X] is developed by [Y] . & 62.8 & 68.0 & 11.3 & 5.4 & 69.2 & 29.4 & 8.8 & 4.9 \\ 
P19 & [X] was born in [Y] . & 21.1 & 21.4 & 3.2 & 0.3 & 19.1 & 5.4 & 6.4 & 6.2 \\ 
P190 & [X] and [Y] are twin cities . & 2.4 & 3.1 & 1.1 & 2.1 & 3.3 & 2.1 & 2.4 & 2.7 \\ 
P20 & [X] died in [Y] . & 27.9 & 33.8 & 11.4 & 10.2 & 33.5 & 12.7 & 11.6 & 10.3 \\ 
P264 & [X] is represented by music label [Y] . & 9.6 & 45.5 & 37.5 & 37.5 & 48.0 & 37.5 & 37.5 & 37.5 \\ 
P27 & [X] is [Y] citizen . & 0 & 47.1 & 10.0 & 10.0 & 47.4 & 13.4 & 10.1 & 10 \\ 
P276 & [X] is located in [Y] . & 41.5 & 47.1 & 8.6 & 0.9 & 50.3 & 5.6 & 4.4 & 4.7 \\ 
P279 & [X] is a subclass of [Y] . & 30.7 & 64.7 & 26.2 & 15.9 & 66.8 & 36.9 & 16.0 & 16 \\ 
P30 & [X] is located in [Y] . & 25.4 & 86.3 & 72.3 & 72.3 & 92.6 & 72.3 & 72.3 & 72.3 \\ 
P31 & [X] is a [Y] . & 36.7 & 64.9 & 11.2 & 8.8 & 71.0 & 24.9 & 8.9 & 8.9 \\ 
P36 & The capital of [X] is [Y] . & 62.2 & 61.3 & 11.8 & 0.0 & 63.4 & 0.1 & 0.0 & 0.1 \\ 
P361 & [X] is part of [Y] .' & 23.6 & 46.4 & 6.0 & 6.0 & 47.6 & 7.6 & 6.0 & 6 \\ 
P364 & The original language of [X] is [Y] . & 44.5 & 51.3 & 25.1 & 25.5 & 50.7 & 27.8 & 25.5 & 25.1 \\ 
P37 & The official language of [X] is [Y] . & 54.6 & 58.6 & 17.0 & 17.0 & 62.6 & 16.0 & 17.0 & 17 \\ 
P39 & [X] has the position of [Y] . & 8 & 42.8 & 28.7 & 27.2 & 45.7 & 32.4 & 30.4 & 27.2 \\ 
P407 & [X] was written in [Y] . & 59.2 & 71.0 & 46.4 & 46.4 & 70.7 & 46.4 & 46.4 & 46.4 \\ 
P413 & [X] plays in [Y] position . & 0.5 & 44.0 & 41.6 & 41.7 & 43.3 & 41.7 & 41.7 & 41.7 \\ 
P449 & [X] was originally aired on [Y] . & 20.9 & 36.0 & 31.0 & 31.9 & 35.1 & 32.2 & 29.8 & 32.6 \\ 
P463 & [X] is a member of [Y] . & 67.1 & 64.0 & 45.8 & 2.2 & 61.8 & 60.4 & 56.4 & 2.2 \\ 
P47 & [X] shares border with [Y] . & 13.7 & 22.2 & 0.1 & 0.0 & 18.7 & 0.9 & 1.1 & 0.3 \\ 
P495 & [X] was created in [Y] . & 16.5 & 40.8 & 10.8 & 10.9 & 41.3 & 12.3 & 13.1 & 10.9 \\ 
P527 & [X] consists of [Y] . & 11.1 & 34.8 & 17.3 & 14.4 & 34.1 & 18.0 & 17.4 & 17.4 \\ 
P530 & [X] maintains diplomatic relations with [Y] . & 2.8 & 3.3 & 0.5 & 0.9 & 2.6 & 1.2 & 0.6 & 1.1 \\ 
P740 & [X] was founded in [Y] . & 7.6 & 15.0 & 7.4 & 5.6 & 14.7 & 7.6 & 7.4 & 7.4 \\ 
P937 & [X] used to work in [Y] . & 29.8 & 43.3 & 14.6 & 13.2 & 43.2 & 16.8 & 14.8 & 14.8 \\
        \bottomrule
    \end{tabular}
    }
    \caption{A detailed breakdown of per-relation probing accuracy and control accuracy on the LAMA test set. \textit{Rand. E}: only the input embeddings are randomly initialized. \textit{Rand. M}: all the weights are randomly initialized. Class Prior is the accuracy from predicting the class that appeared most often in the training data. }
    \label{tab:breakdown_full}
\end{table*}


% \begin{table*}[ht]
%     \resizebox{2.\columnwidth}{!}{%
%     \begin{tabular}{l | lc | ccc | ccc}
%         \toprule
%         \multirow{2}{*}{\tf{Relation}} &  \multicolumn{2}{c|}{{\bf LAMA (manual prompts)}} & \multicolumn{3}{c|}{{\bf \ours}} & \multicolumn{3}{c}{{\bf \finetuning}} \\
%          & Prompt & Acc & Acc & Rand E. & Rand M. & Acc & Rand E. & Rand M.\\
%         \midrule

% P1001 & [X] is a legal term in [Y] . & 70.47 & 85.45 & 50.36 & 9.42 & 85.45 & 53.92 & 9.56 \\
% P101 & [X] works in the field of [Y] . & 9.91 & 13.36 & 8.91 & 10.06 & 15.23 & 11.49 & 10.78 \\
% P103 & The native language of [X] is [Y] . & 72.16 & 85.77 & 59.98 & 59.98 & 87.31 & 63.66 & 60.08 \\
% P106 & [X] is a [Y] by profession . & 0.63 & 36.95 & 29.96 & 20.67 & 33.40 & 29.12 & 25.57 \\
% P108 & [X] works for [Y] . & 6.79 & 9.66 & 7.31 & 7.31 & 10.44 & 7.31 & 7.83 \\
% P127 & [X] is owned by [Y] . & 34.79 & 51.38 & 7.13 & 10.19 & 52.55 & 17.18 & 14.70 \\
% P1303 & [X] plays [Y] . & 7.59 & 24.87 & 22.76 & 22.34 & 24.87 & 22.76 & 22.76 \\
% P131 & [X] is located in [Y] . & 23.27 & 39.61 & 0.57 & 1.59 & 40.52 & 1.82 & 0.57 \\
% P136 & [X] plays [Y] music . & 0.75 & 64.77 & 55.42 & 55.42 & 62.62 & 54.78 & 55.42 \\
% P1376 & [X] is the capital of [Y] . & 73.93 & 62.66 & 0.86 & 0.00 & 66.52 & 0.00 & 0.43 \\
% P138 & [X] is named after [Y] . & 61.55 & 74.61 & 0.94 & 0.47 & 73.83 & 35.36 & 1.56 \\
% P140 & [X] is affiliated with the [Y] religion . & 0.63 & 77.59 & 53.70 & 53.70 & 80.13 & 53.70 & 53.70 \\
% P1412 & [X] used to communicate in [Y] . & 65.02 & 76.78 & 25.39 & 20.64 & 76.06 & 27.35 & 26.73 \\
% P159 & The headquarter of [X] is in [Y] . & 32.37 & 37.54 & 9.00 & 9.00 & 37.54 & 9.31 & 9.00 \\
% P17 & [X] is located in [Y] . & 31.29 & 57.85 & 3.12 & 2.37 & 58.28 & 7.42 & 2.69 \\
% P176 & [X] is produced by [Y] . & 85.64 & 87.15 & 8.94 & 8.94 & 90.13 & 82.63 & 68.35 \\
% P178 & [X] is developed by [Y] . & 62.84 & 68.70 & 8.63 & 4.74 & 61.59 & 33.67 & 8.12 \\
% P19 & [X] was born in [Y] . & 21.08 & 20.45 & 5.61 & 5.61 & 18.86 & 4.45 & 6.25 \\
% P190 & [X] and [Y] are twin cities . & 2.41 & 3.13 & 2.62 & 1.31 & 3.13 & 2.52 & 2.12 \\
% P20 & [X] died in [Y] . & 27.91 & 33.26 & 10.49 & 10.91 & 33.16 & 12.80 & 13.22 \\
% P264 & [X] is represented by music label [Y] . & 9.56 & 47.09 & 37.53 & 37.53 & 50.35 & 37.53 & 37.53 \\
% P27 & [X] is [Y] citizen . & 0.00 & 47.10 & 10.04 & 4.97 & 49.38 & 11.49 & 10.04 \\
% P276 & [X] is located in [Y] . & 41.50 & 47.18 & 5.01 & 4.49 & 49.37 & 5.12 & 4.91 \\
% P279 & [X] is a subclass of [Y] . & 30.74 & 66.04 & 28.11 & 15.98 & 66.36 & 42.84 & 15.98 \\
% P30 & [X] is located in [Y] . & 25.44 & 89.54 & 72.31 & 72.31 & 92.41 & 72.31 & 72.31 \\
% P31 & [X] is a [Y] . & 36.66 & 65.73 & 8.89 & 8.68 & 69.09 & 28.53 & 9.00 \\
% P36 & The capital of [X] is [Y] . & 62.16 & 61.97 & 0.00 & 0.00 & 62.82 & 0.57 & 0.00 \\
% P361 & [X] is part of [Y] .' & 23.61 & 46.78 & 6.01 & 6.01 & 48.50 & 7.40 & 6.01 \\
% P364 & The original language of [X] is [Y] . & 44.51 & 50.00 & 24.88 & 19.74 & 51.87 & 26.99 & 25.58 \\
% P37 & The official language of [X] is [Y] . & 54.55 & 61.39 & 16.98 & 16.98 & 64.70 & 18.01 & 16.98 \\
% P39 & [X] has the position of [Y] . & 7.96 & 43.39 & 31.39 & 31.39 & 42.15 & 33.74 & 29.48 \\
% P407 & [X] was written in [Y] . & 59.18 & 70.13 & 46.41 & 46.64 & 72.06 & 46.41 & 46.41 \\
% P413 & [X] plays in [Y] position . & 0.53 & 43.80 & 41.70 & 41.70 & 41.70 & 41.70 & 41.70 \\
% P449 & [X] was originally aired on [Y] . & 20.89 & 35.23 & 29.66 & 32.50 & 35.23 & 26.82 & 29.21 \\
% P463 & [X] is a member of [Y] . & 67.11 & 62.67 & 38.22 & 2.22 & 62.22 & 59.11 & 57.33 \\
% P47 & [X] shares border with [Y] . & 13.67 & 22.28 & 0.00 & 0.00 & 21.85 & 0.44 & 1.09 \\
% P495 & [X] was created in [Y] . & 16.50 & 40.37 & 10.89 & 11.88 & 39.82 & 14.08 & 13.09 \\
% P527 & [X] consists of [Y] . & 11.07 & 34.84 & 17.42 & 8.61 & 35.35 & 11.78 & 17.11 \\
% P530 & [X] maintains diplomatic relations with [Y] . & 2.81 & 3.31 & 0.40 & 0.60 & 2.91 & 2.41 & 0.70 \\
% P740 & [X] was founded in [Y] . & 7.59 & 16.67 & 7.37 & 7.37 & 16.03 & 7.27 & 7.37 \\
% P937 & [X] used to work in [Y] . & 29.77 & 44.44 & 14.78 & 14.78 & 44.55 & 17.40 & 14.78 \\

%         \bottomrule
%     \end{tabular}
%     }
%     \caption{A detailed breakdown of per-relation probing accuracy and control accuracy on the LAMA test set. \textit{Rand. E}: only the input embeddings are randomly initialized. \textit{Rand. M}: all the weights are randomly initialized. }
%     \label{tab:breakdown_full}
% \end{table*}


==> tables/control_result.tex <==
%!TEX root = ../main.tex

\begin{table}
    \centering
    \resizebox{1.0\columnwidth}{!}{%
    \begin{tabular}{cc| cc | cc | cc}
        \toprule
         &  & \multicolumn{2}{c|}{\tf{Pre-T.}} & \multicolumn{2}{c|}{\tf{Rand E.}} & \multicolumn{2}{c}{\tf{Rand M.}} \\
        \tf{Method} & \tf{Type} & Maj. & All & Maj. & All & Maj. & All \\
        % \midrule
        % \multirow{4}{*}{Majority}
        %  & 1-1 & 1.8 & - & - \\
        %  & N-1 & 23.9 & - & - \\
        %  & N-M & 22.0 & - & - \\
        %  & All & 22.0 & - & - \\
        \midrule
\multirow{4}{*}{\shortstack{\autop \\ (5 {\tv}s)}} & 1-1 & 0.2 & 58.0 & 0.0 & 0.1 & 0.0 & 0.0 \\
 & N-1 & 18.8 & 46.5 & 6.7 & 6.7 & 0.0 & 0.0 \\
 & N-M & 8.0 & 34.0 & 0.2 & 0.8 & 0.0 & 0.0 \\
 & All & 13.7 & 42.2 & 3.8 & 4.0 & 0.0 & 0.0 \\
\midrule
\multirow{4}{*}{\shortstack{\ours \\ (manual)}} & 1-1 & 0.0 & 59.0 & 0.0 & 5.9 & 0.0 & 0.0 \\
 & N-1 & 21.5 & 53.7 & 22.2 & 23.6 & 22.3 & 22.6 \\
 & N-M & 8.5 & 40.0 & 9.0 & 17.5 & 8.7 & 10.1 \\
 & All & 15.4 & 48.6 & 16.0 & 20.3 & 15.9 & 16.6 \\
\midrule
\multirow{4}{*}{Fine-tune} & 1-1 & 0.2 & 63.0 & 0.0 & 0.1 & 0.0 & 0.0 \\
 & N-1 & 19.5 & 54.7 & 22.0 & 30.4 & 22.4 & 26.1 \\
 & N-M & 8.2 & 40.2 & 8.3 & 22.2 & 9.0 & 16.1 \\
 & All & 14.2 & 49.4 & 15.5 & 25.8 & 16.1 & 21.0 \\
        \bottomrule
    \end{tabular}
    }
    \vspace{-0.4em}
    \caption{
    %Probing results on LAMA using the BERT-base-cased model. {Pre-T.}: pre-trained models. {Rand. E}: only the input embeddings are randomly initialized. {Rand. M}: all the weights are randomly initialized.
    Optimized prompts can elicit many LAMA facts from randomly initialized Transformers by exploiting both class statistics and other lexical regularities.
    \ti{All} gives the accuracy on LAMA, averaged over relations. \ti{Maj.} shows how much of this accuracy can be attributed to the majority class prior: for each test example $\langle s, r, o \rangle$, the \ti{Maj.} score is defined as $\mathbbm{1}[\hat{o} = \tilde{o}_r = o]$, where $\hat{o}$ is the predicted label and $\tilde{o}_r$ is the training class majority label for relation $r$.
    % \dan{I'm going to replace the numbers in this table with an ``attribution'' score: in each setting, what \% of the correct predictions can be attributed to the class prior? This will  show that optimized prompts can exploit lexical regularities in addition to simple class statistics.}
    }
    \label{tab:control_results}
    \vspace{-1em}
\end{table}

% \begin{table}
%     \centering
%     \resizebox{1.0\columnwidth}{!}{%
%     \begin{tabular}{cc|rrr}
%         \toprule
%         \tf{Method} & \tf{Type} & \tf{Pre-T.} & \tf{Rand E.} & \tf{Rand M.} \\
%         % \midrule
%         % \multirow{4}{*}{Majority}
%         %  & 1-1 & 1.8 & - & - \\
%         %  & N-1 & 23.9 & - & - \\
%         %  & N-M & 22.0 & - & - \\
%         %  & All & 22.0 & - & - \\
%         \midrule
%         \multirow{4}{*}{\shortstack{\autop \\ (5 {\tv}s) }}
%          & 1-1 & 40.2 & 0.1 & 0.0 \\
%          & N-1 & 48.5 & 6.7 & 0.0\\
%          & N-M & 34.0 & 0.7 & 0.0\\
%          & All & 42.9 & 4.0 & 0.0 \\
%          \midrule
%          \multirow{4}{*}{\shortstack{\ours \\ (w/ manual)}}
%          & 1-1 & 59.6 & 5.9 & 0.0\\
%          & N-1 & 54.1 & 23.8 & 22.6\\
%          & N-M & 40.1 & 17.5 & 10.1 \\
%          & All & 48.6 & 20.5 & 16.6 \\
%          \midrule
%          \multirow{4}{*}{\shortstack{\finetuning \\ (|\rset| models)}}
%          & 1-1 & 63.0 & 0.1 & 0.0\\
%          & N-1 & 54.6 & 30.4 & 26.1\\
%          & N-M & 40.3 & 22.2 & 16.1\\
%          & All & 49.4 & 25.8 & 21.0 \\
%         %  \midrule
%         %  \multirow{4}{*}{\shortstack{\finetuning \\ (one model)}}
%         %  & 1-1 & 61.2 & 0.0 & 0.0\\
%         %  & N-1 & 52.5 & 6.6 & 7.1\\
%         %  & N-M & 39.4 & 1.0 & 5.5\\
%         %  & All & 47.8 & 6.1 & 4.1 \\
%         \bottomrule
%     \end{tabular}
%     }
%     \vspace{-0.4em}
%     \caption{
%     %Probing results on LAMA using the BERT-base-cased model. {Pre-T.}: pre-trained models. {Rand. E}: only the input embeddings are randomly initialized. {Rand. M}: all the weights are randomly initialized.
%     \dan{I'm going to replace the numbers in this table with an ``attribution'' score: in each setting, what \% of the correct predictions can be attributed to the class prior? This will  show that optimized prompts can exploit lexical regularities in addition to simple class statistics.}
%     }
%     \label{tab:control_results}
%     \vspace{-1em}
% \end{table}


% \begin{table*}
%     \centering
%     \resizebox{2.0\columnwidth}{!}{%
%     \begin{tabular}{l | cc | cccc | cccc }
%         \toprule
%         & \multicolumn{2}{c|}{\tf{Pre-trained model}} &  \multicolumn{4}{c|}{\tf{Ctrl: random embeddings}} & \multicolumn{4}{c}{\tf{Ctrl: random model}} \\
%         \tf{Method} & acc & entropy & acc & entropy & $\Delta$acc & $\mathcal{G}$ & acc & entropy & $\Delta$acc & $\mathcal{G}$ \\
%         \midrule
%         Majority & 22.0 & - & 22.0 & - & 0.0 & - & 22.0 & - & 0.0 & -  \\
%         \midrule
%         \lama~(manual) & 31.1 & 3.90 & 0.0 & 10.28 & 31.1 & 6.38 & 0.0 & 10.08 & 31.1 & 6.18 \\
%         \lpaqa & 34.1 & 3.67 & 0.0 & 10.02 & 34.1 & 6.35 & 0.0 & 9.89 & 34.1 & 6.22 \\
%         \autop & 42.9 & 2.92 & 4.0 & 9.45 & 28.9 & 6.53 & 0.0 & 9.97 & 42.9 & 7.05 \\
%         \midrule
%         {\ours} & 49.1 & 2.39 & 20.0 & 7.52 & 29.1 & 5.13 & 17.1 & 8.92 & 32.0 & 6.53 \\
%         \midrule
%         \finetuning~($|R|$ models) & 49.5 & 2.38  & 25.4 & 5.44 & 24.1 & 3.06  & 20.9 & 6.85 & 28.6 & 4.47 \\
%         \finetuning~(one model) & 47.8 & 2.68  & 6.1 & 6.87 & 41.7 & 4.19 & 4.1 & 7.04 & 43.7 & 4.36 \\
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Probing results on TRE-x using the BERT-base-cased model. The performance of contorl tasks are based on a randomly initialized BERT.}
%     \label{tab:control_results}
% \end{table*}



% \begin{table*}
%     \centering
%     \resizebox{2.0\columnwidth}{!}{%
%     \begin{tabular}{l | cc | cc | cc }
%         \toprule
%         & \multicolumn{2}{c}{BERT} & \multicolumn{2}{c}{Random BERT} & \multicolumn{2}{c}{Information Gain} \\
%         Method & Accuracy & $H_{q_{\theta}}(S, O \mid M)$ & Accuracy & $H_{q_{\theta'}}(S, O \mid \mathbf{c}(M))$ & Accuracy & $\mathcal{G}$ \\
%         \midrule
%         Majority & 22.0 & - & 22.0 & - & 0.0 & - \\
%         \midrule
%         \lama (manual) & 31.1 & 3.90 & TODO & TODO &  &  \\
%         \lpaqa & 34.1 & TODO & TODO & TODO &  &  \\
%         \autop & 42.9 & 2.92 & TODO & TODO &  &  \\
%         \midrule
%         \ours~(5 \vv s) & 48.2 & 2.36 & 17.1 & 8.98 & 31.1 & \\
%         \ours~(10 \vv s) & 48.4 & 2.37 & 17.6 & 8.85 & 30.8 & \\
%         \ours~(init. w/ manual) & 49.1 & 2.39 & 17.1 & 8.92 & 32.0 & \\
%         \midrule
%         \finetuning~(\subj \mask) & 48.1 & 2.42 & 21.7 & 6.52 & 26.4 & \\
%         \finetuning~(manual) & 49.5 & 2.38 & 20.9 & 6.85 & 28.6 &  \\
%         \finetuning~(manual, one model for all) & 47.8 & 2.68 & \\
%         \bottomrule
%         % \lpaqa & 59.8 & 35.9 & 27.9 & 34.1 & & & & 28.7\\
%         % \autop & 40.2 & 48.5 & 34.0 & 42.9 & & \\
%         % \midrule
%         % \ours~(5 \vv s) & 45.9 & 53.4 & 40.1 & 48.2 & 21.3 & 24.8 & 17.1 & 37.5  \\
%         % \ours~(10 \vv s) & 52.4 & 53.7 & 39.6 & 48.4 & 22.9 & 25.4 & 17.6 & 37.9  \\
%         % \ours~(init. w/ manual) & 62.0 & 54.1 & \tf{40.2} & {49.1} & 20.0 & 24.2 & 17.1 & 38.4  \\
%         % \midrule
%         % \finetuning~(\subj \mask)  & 48.5 & 53.9 & 39.1 & 48.1 & 25.0 & 26.9 & 21.7 & 38.2  \\
%         % \finetuning~(\subj \mask, freezing input)  & TODO & TODO & TODO & TODO & TODO & TODO & & TODO \\
%         % \finetuning~(manual) & \tf{62.8} & \tf{54.9} & 39.9 & \tf{49.5} & 25.4 & 27.5 & 20.9 & \tf{39.5}  \\
%         % \finetuning~(manual, freezing input) & 61.3 & 54.7 & 40.1 & 49.3 & 25.6 & 27.4 & 20.8 & 39.8  \\
%         % \bottomrule
%     \end{tabular}
%     }
%     \caption{Probing results on TRE-x using the BERT-base-cased model. The performance of contorl tasks are based on a randomly initialized BERT.
%     \zexuan{Notations need to be changed.} \zexuan{Should we include breakdown accuracy (1-1, N-1, etc.) here?}}
%     \label{tab:lama_results}
% \end{table*}
%


==> tables/entity_typing_result.tex <==
%!TEX root = ../main.tex

\begin{table}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{lccc}
        \toprule
        Method & BERT & RoBERTa & ALBERT \\
        \# & (110M) & (330M) & (235M)$\dagger$ \\
        \midrule
        Entity only &  \\
        Context only &  \\
        Full & \\
        \bottomrule
    \end{tabular}
    }
    \caption{Results of different pre-trained LMs on Open Entity leveraging different information.}
    \label{tab:entity_typing}
\end{table}


==> tables/majority_class.tex <==
%!TEX root = ../main.tex


\begin{table}
    \centering
    \resizebox{1.0\columnwidth}{!}{%
    \begin{tabular}{l l | r r |rrr}
        \toprule
Relation & Maj. class & Train \% & Test \% & Auto & Opti & FT \\
\midrule
% genre & jazz & 46.9 & 55.4 & \tf{98.4} & 79.1 & 67.8 \\
% religion & Islam & 76.1 & 53.7 & \tf{92.2} & 67.0 & 57.9 \\
% position played & midfielder & 69.2 & 41.7 & 98.8 & 93.1 & \tf{99.5} \\
% occupation & politician & 26.9 & 14.3 & \tf{96.5} & 42.9 & 50.1 \\
% employer & IBM & 30.3 & 7.8 & \tf{98.2} & 52.0 & 36.8 \\
% instrument & piano & 25.6 & 22.8 & \tf{97.9} & 82.5 & 78.8 \\
% position held & bishop & 42.8 & 27.2 & \tf{100.0} & 71.9 & 51.7 \\
religion & Islam & 76.1 & 53.7 & \tf{92.2} & 73.6 & 63.4 \\
position played & midfielder & 69.2 & 41.7 & \tf{98.8} & 89.2 & 92.6 \\
genre & jazz & 46.9 & 55.4 & \tf{98.4} & 78.0 & 68.3 \\
position held & bishop & 42.8 & 27.2 & \tf{100.0} & 54.1 & 46.4 \\
employer & IBM & 30.3 & 7.8 & \tf{98.2} & 41.0 & 46.5 \\
occupation & politician & 26.9 & 14.3 & \tf{96.5} & 40.4 & 50.9 \\
instrument & piano & 25.6 & 22.8 & \tf{97.9} & 80.1 & 79.8 \\
        \bottomrule
    \end{tabular}
    }
    \vspace{-0.4em}
    \caption{How often does each prompt return the training-set majority class label?
    %\zexuan{TODO: update Opti and FT}
    \zexuan{The size of the table doesn't look good?}
    }
    \label{tab:majority_class}
    \vspace{-1em}
\end{table}

==> tables/majority_class_details.tex <==
\begin{table*}
    \resizebox{2.\columnwidth}{!}{%
    \begin{tabular}{llll | rr | rrrr }
        \toprule
\tf{Relation} & \tf{Type} & \tf{Name} & \tf{Maj. label} & \tf{Train \%} & \tf{Test \%} & \tf{Manual} & \tf{LPAQA} & \tf{Auto} & \tf{Opti} \\
        \midrule
P1376 & 1-1 & capital of & Japan & 2.8 & 0.4 & 0.4 & 0.0 & 0.4 & 0.0 \\
P36 & 1-1 & capital & Marseille & 5.3 & 0.0 & 0.1 & 0.1 & 0.0 & 0.1 \\
P103 & N-1 & native language & French & 61.8 & 60.1 & 45.5 & 45.5 & 63.5 & 63.1 \\
P127 & N-1 & owned by & Germany & 10.7 & 6.8 & 0.3 & 7.9 & 9.8 & 7.7 \\
P131 & N-1 & located in... & Karnataka & 4.2 & 0.6 & 0.1 & 0.2 & 0.0 & 2.2 \\
P136 & N-1 & genre & jazz & 46.9 & 55.4 & 0.6 & 10.2 & 98.4 & 79.3 \\
P138 & N-1 & named after & Peter & 6.0 & 1.6 & 0.3 & 0.2 & 0.3 & 0.5 \\
P140 & N-1 & religion & Islam & 76.1 & 53.7 & 0.0 & 48.6 & 92.2 & 67.4 \\
P159 & N-1 & headquarters location & London & 7.9 & 9.0 & 11.5 & 21.3 & 38.7 & 32.5 \\
P17 & N-1 & country & Iran & 9.9 & 2.8 & 1.6 & 0.8 & 3.3 & 6.6 \\
P176 & N-1 & manufacturer & Honda & 20.4 & 8.9 & 8.3 & 7.9 & 8.4 & 8.9 \\
P19 & N-1 & place of birth & London & 3.4 & 6.2 & 24.0 & 24.0 & 25.8 & 23.5 \\
P20 & N-1 & place of death & Paris & 8.5 & 10.3 & 21.3 & 21.3 & 15.2 & 11.9 \\
P264 & N-1 & record label & Motown & 34.2 & 37.5 & 0.9 & 2.1 & 0.7 & 77.6 \\
P276 & N-1 & location & London & 4.6 & 4.7 & 4.7 & 4.7 & 15.1 & 14.9 \\
P279 & N-1 & subclass of & protein & 15.8 & 16.0 & 0.0 & 5.1 & 11.7 & 15.5 \\
P30 & N-1 & continent & Antarctica & 95.6 & 72.3 & 24.6 & 13.8 & 82.9 & 81.1 \\
P361 & N-1 & part of & Andes & 66.6 & 6.0 & 0.0 & 0.1 & 0.1 & 17.0 \\
P364 & N-1 & original language... & English & 15.0 & 25.1 & 45.6 & 60.5 & 52.6 & 42.9 \\
P37 & N-1 & official language & Finnish & 48.0 & 17.0 & 7.7 & 9.7 & 31.8 & 23.6 \\
P407 & N-1 & language of work... & English & 30.6 & 46.4 & 49.5 & 51.8 & 62.9 & 54.8 \\
P413 & N-1 & position played... & midfielder & 69.2 & 41.7 & 0.6 & 31.1 & 98.8 & 89.2 \\
P449 & N-1 & original network & NBC & 33.1 & 32.6 & 2.6 & 1.0 & 36.9 & 89.4 \\
P495 & N-1 & country of origin & Canada & 14.8 & 10.9 & 0.8 & 1.2 & 5.8 & 42.0 \\
P740 & N-1 & location of formation & London & 8.8 & 7.4 & 20.7 & 36.0 & 68.2 & 71.5 \\
P1001 & N-M & applies to jurisdiction & Canada & 10.0 & 9.6 & 9.6 & 13.4 & 10.0 & 10.6 \\
P101 & N-M & field of work & physics & 11.0 & 10.8 & 0.6 & 4.2 & 30.7 & 34.3 \\
P106 & N-M & occupation & politician & 26.9 & 14.3 & 0.0 & 0.0 & 96.5 & 42.7 \\
P108 & N-M & employer & IBM & 30.3 & 7.8 & 31.3 & 24.3 & 98.2 & 49.3 \\
P1303 & N-M & instrument & piano & 25.6 & 22.8 & 5.4 & 35.1 & 97.9 & 97.4 \\
P1412 & N-M & languages spoken... & French & 21.2 & 20.6 & 15.9 & 18.6 & 18.9 & 20.7 \\
P178 & N-M & developer & Sega & 29.2 & 4.9 & 2.0 & 0.8 & 25.0 & 17.6 \\
P190 & N-M & twinned admin... & Moscow & 2.8 & 2.6 & 4.7 & 4.6 & 17.6 & 14.0 \\
P27 & N-M & country of citizenship & Canada & 10.1 & 10.0 & 0.0 & 16.0 & 1.9 & 14.9 \\
P31 & N-M & instance of & album & 24.5 & 8.9 & 0.0 & 0.0 & 5.5 & 18.1 \\
P39 & N-M & position held & bishop & 42.8 & 27.2 & 9.5 & 50.9 & 100.0 & 54.1 \\
P463 & N-M & member of & UNESCO & 30.2 & 2.2 & 0.0 & 0.0 & 7.1 & 15.1 \\
P47 & N-M & shares border with & Lyon & 1.0 & 0.2 & 0.0 & 0.0 & 0.0 & 0.1 \\
P527 & N-M & has part & carbon & 10.9 & 17.4 & 1.4 & 0.1 & 10.2 & 28.4 \\
P530 & N-M & diplomatic relation & Greece & 2.3 & 1.1 & 0.1 & 0.6 & 6.2 & 6.2 \\
P937 & N-M & work location & London & 17.1 & 14.8 & 29.7 & 27.3 & 20.4 & 24.7 \\
        \bottomrule
    \end{tabular}
    }
    \caption{The percentage of time that each model predicts the training class majority label for each relation type when evaluated on the LAMA benchmark. The Train \% and Test \% columns show the percentage of facts that are labeled with the training majority label in the training set (collected from Wikidata by~\citealp{shin2020autoprompt}) and in the LAMA benchmark respectively. (Note that LPAQA prompts are tuned on a different collection of Wikidata training examples.)}
    \label{tab:majority_class_details}
\end{table*}

==> tables/one_vs_all_relations.tex <==
%!TEX root = ../main.tex

\begin{table}
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{l c}
        \toprule
        Method & Acc \\
        \midrule
        \ours~(one prompt per relation) & 49.1 \\
        \midrule
        \finetuning~(one model per relation)  & 49.5 \\
        \finetuning~(one model for all) & 47.8 \\
        \bottomrule
    \end{tabular}
    }
    \caption{Comparison of having one model per relaion vs one model for all relations. \todo{Can we this table to freezing input too? Sorry for extra work.} \dan{Could we train one-model-for-all on the control? Then we could merge this with Table~\ref{tab:lama_results}}} 
    \label{table:one_vs_all}
\end{table}


==> tables/performance.tex <==
%!TEX root = ../main.tex

\begin{table}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{l|ccc}
        \toprule
        Method & Time & Memory & $\mathcal{G}$\\
        \midrule
        {\lpaqa} \\
        {\autop} \\
        {\ours} \\
        {\finetuning} ($|R|$ models) \\
        {\finetuning} (one model) \\
        \bottomrule
    \end{tabular}
    }
    \caption{We compare the performance costs of different prompt-finding methods in terms of training time (seconds per relation, until convergence) and memory (MB per prompt), along with information gain relative to the control.}
    \label{tab:performance}
\end{table}


==> tables/semirandom.tex <==
%!TEX root = ../main.tex

\begin{table}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{l | cc | cc | cc }
        \toprule
        & \multicolumn{2}{c}{BERT} & \multicolumn{2}{c}{Random BERT} & \multicolumn{2}{c}{Information Gain} \\
        Method & Accuracy & $H_{q_{\theta}}(S, O \mid M)$ & Accuracy & $H_{q_{\theta'}}(S, O \mid \mathbf{c}(M))$ & Accuracy & $\mathcal{G}$ \\
        \midrule
        All \\
        {\autop} \\
        {\ours} \\
        {\finetuning} \\
        \bottomrule
    \end{tabular}
    }
    \caption{\dan{I haven't filled this out yet} Accuracy and gain with a partly reinitialized version of BERT: BERT has all of the parameters from pre-training but we reinitialize the token embeddings.}
    \label{tab:semirandom}
\end{table}


==> tables/tacred_result.tex <==
%!TEX root = ../main.tex

\begin{table}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{lcccc}
        \toprule
        Method & BERT & BERT & RoBERTa & ALBERT \\
        \# & (110M) & (330M) &(330M) & (235M)$\dagger$ \\
        \midrule
        Entity only & 45.1 & 47.0 & 49.2 & 46.4 \\
        Context only & 58.5 & 62.3 & 59.3 & 58.1 \\
        Full & 67.1 & 70.2 & 67.2 & 63.6 \\
        \bottomrule
    \end{tabular}
    }
    \caption{Results of different pre-trained LMs on TACRED leveraging different information. Entities: \ttt{Billy Mays [SEP] Tampa}; Context: \ttt{[E1] died at his home in [E2]}; Full: \ttt{Billy Mays died at his home in Tampa}. \danqi{Here I am expecting to see that 1) Entity only is consistent with probing results; 2) different models can have different entity-only and context-only results; 3) This can help us decide how to choose pre-trained models in factual knowledge related downstream tasks.} \zexuan{RoBERTa and ALBERT performs worse than BERT on Context only. I suspect it is because I didn't tune hyper-parameters for these two models.}}
    \label{tab:tacred_results}
\end{table}


==> tables/training_data.tex <==
%!TEX root = ../main.tex

\begin{table*}
    \resizebox{2.1\columnwidth}{!}{%
    \begin{tabular}{lccccc}
        \toprule
        Method & 1k(AutoPrompt) & 1k(ours) & 10k(ours) & 1k(ours,hard) & 10k (ours,hard) \\
        \midrule
        Manual & 31.1 \\
        AutoPrompt & 42.9  \\
        OptPrompt & 48.2 \\
        OptPrompt (init w/ LAMA) & 49.1 & 48.7 & 49.3 & 47.0 & 47.4  \\
        Fine-tuning ([x] [y]) & 48.1 & \\
        Fine-tuning (w/ LAMA templates) & 49.5 & 49.1 & 49.9 & 47.1 & 48.3 \\
        \bottomrule
    \end{tabular}
    }
    \caption{Comparison of different training data. \danqi{The point of this table is to see 1) whether increasing training data makes a difference; 2) If we constrain that the model can't obtain relevant knowledge from the training data, would the performance drop a lot? } \zexuan{the table needs to be reformed. hard: we require the training triples' subject tokens have no overlap with the evaluation triples' subject tokens.}}
    \label{tab:training_data}
\end{table*}

